Internet Sanctions on Russian Media: Actions and Effects

As a response to the Russian aggression against Ukraine, the European Union (EU), through the notion of "digital sovereignty", imposed sanctions on organizations and individuals affiliated with the Russian Federation that prohibit broadcasting content, including online distribution. In this paper, we interrogate the implementation of these sanctions and interpret them as a means to translate the union of states' governmental edicts into effective technical countermeasures. Through longitudinal traffic analysis, we construct an understanding of how ISPs in different EU countries attempted to enforce these sanctions, and compare these implementations to similar measures in other western countries. We find a wide variation of blocking coverage, both internationally and within individual member states. We draw the conclusion that digital sovereignty through sanctions in the EU has a concrete but distinctly limited impact on information flows.

==> tables/eduvpn_dns_anomalies.tex <==
\begin{table}[H]
    \caption{DNS anomalies observed during the domain name resolution with the recursive resolvers of the corresponding networks as announced on DHCP.}
    \label{tbl:eduvpn-dns-anomalies}
    \centering
    \begin{tabular}{lcc}
        \hline
        Domain Name         & Germany            & The Netherlands   \\
        \hline
        actualidad.rt.com.  & \texttt{NXDOMAIN}  & \texttt{SERVFAIL} \\
        de.rt.com.          & \texttt{NXDOMAIN}  & \texttt{SERVFAIL} \\
        deutsch.rt.com.     & \texttt{NXDOMAIN}  & \texttt{SERVFAIL} \\
        fr.rt.com.          & \texttt{NXDOMAIN}  & \texttt{SERVFAIL} \\
        francais.rt.com.    & \texttt{NXDOMAIN}  & \texttt{SERVFAIL} \\
        radiosputnik.ria.ru. & \texttt{NXDOMAIN} & -        \\
        rt.com.             & \texttt{NXDOMAIN}  & \texttt{SERVFAIL} \\
        snanews.de.         & -         & \texttt{SERVFAIL} \\
        www.rt.com.         & \texttt{NXDOMAIN} & \texttt{SERVFAIL}  \\
        www.sputniknews.com. & \texttt{NXDOMAIN} & \texttt{SERVFAIL} \\
        \hline
    \end{tabular}
\end{table}


==> tables/eduvpn_secure_internet_access_overview.tex <==
\begin{table}[H]
    \caption{EduVPN Secure Internet Access sites and the DNS resolver announced via DHCP.}
    \label{tbl:eduvpn-secure-internet-access-overview}
    \centering
    \begin{tabular}{cllrlc}
        \hline
        Country      & Region   & DNS Resolver \\
        \hline
        AL           & RIPE     & Quad9        \\
        DE           & RIPE     & local        \\
        DK           & RIPE     & local        \\
        FI           & RIPE     & local        \\
        KE           & AFRINIC  & local        \\
        LK           & APNIC    & Quad9        \\
        MY           & APNIC    & Quad9        \\
        NL           & RIPE     & local        \\
        PK           & APNIC    & Google       \\
        UG           & AFRINIC  & local        \\
        ZA           & AFRINIC  & Quad9        \\
        \hline
    \end{tabular}
\end{table}


==> tables/ripe_atlas_dns_at.tex <==
\definecolor{0}{rgb}{0.267004,0.004874,0.329415} 
\definecolor{1}{rgb}{0.282656,0.100196,0.42216} 
\definecolor{2}{rgb}{0.277134,0.185228,0.489898} 
\definecolor{3}{rgb}{0.253935,0.265254,0.529983} 
\definecolor{4}{rgb}{0.221989,0.339161,0.548752} 
\definecolor{5}{rgb}{0.190631,0.407061,0.556089} 
\definecolor{6}{rgb}{0.163625,0.471133,0.558148} 
\definecolor{7}{rgb}{0.139147,0.533812,0.555298} 
\definecolor{8}{rgb}{0.120565,0.596422,0.543611} 
\definecolor{9}{rgb}{0.134692,0.658636,0.517649} 
\definecolor{10}{rgb}{0.20803,0.718701,0.472873} 
\definecolor{11}{rgb}{0.327796,0.77398,0.40664} 
\definecolor{12}{rgb}{0.477504,0.821444,0.318195} 
\definecolor{13}{rgb}{0.647257,0.8584,0.209861} 
\definecolor{14}{rgb}{0.82494,0.88472,0.106217} 
\definecolor{15}{rgb}{0.993248,0.906157,0.143936} 
\begin{table} 
\setlength\tabcolsep{1pt} 
\caption{Share of uncensored DNS responses for probes using ISP resolvers in Austria for mirror pages of the German site of RT.}\label{tbl:blocking_at} 
\centering 
\scriptsize 
\adjustbox{max width=\textwidth}{% 
\begin{tabular}{l c c c c c c c } 
 & \DomainHead{2022-08-01} & \DomainHead{2022-09-08} & \DomainHead{2022-10-31} & \DomainHead{2023-02-10} & \DomainHead{2023-04-19} & \DomainHead{2023-07-26} & \DomainHead{2023-09-01} \\ \midrule 
 rtde.site & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{4} \color{white} 25 & \cellcolor{1} \color{white} 12 & \cellcolor{3} \color{white} 24 & \cellcolor{2} \color{white} 14 \\ 
 rtde.team & \cellcolor{15} 100 & \cellcolor{15} 95 & \cellcolor{15} 100 & \cellcolor{4} \color{white} 25 &  & \cellcolor{4} \color{white} 31 & \cellcolor{0} \color{white} 0 \\ 
 test.rtde.live & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{4} \color{white} 26 &  & \cellcolor{4} \color{white} 29 & \cellcolor{3} \color{white} 22 \\ 
\bottomrule
\end{tabular}}
\end{table}

==> tables/ripe_atlas_dns_overblocking.tex <==
\definecolor{0}{rgb}{0.267004,0.004874,0.329415} 
\definecolor{1}{rgb}{0.282656,0.100196,0.42216} 
\definecolor{2}{rgb}{0.277134,0.185228,0.489898} 
\definecolor{3}{rgb}{0.253935,0.265254,0.529983} 
\definecolor{4}{rgb}{0.221989,0.339161,0.548752} 
\definecolor{5}{rgb}{0.190631,0.407061,0.556089} 
\definecolor{6}{rgb}{0.163625,0.471133,0.558148} 
\definecolor{7}{rgb}{0.139147,0.533812,0.555298} 
\definecolor{8}{rgb}{0.120565,0.596422,0.543611} 
\definecolor{9}{rgb}{0.134692,0.658636,0.517649} 
\definecolor{10}{rgb}{0.20803,0.718701,0.472873} 
\definecolor{11}{rgb}{0.327796,0.77398,0.40664} 
\definecolor{12}{rgb}{0.477504,0.821444,0.318195} 
\definecolor{13}{rgb}{0.647257,0.8584,0.209861} 
\definecolor{14}{rgb}{0.82494,0.88472,0.106217} 
\definecolor{15}{rgb}{0.993248,0.906157,0.143936} 
\begin{table} 
\setlength\tabcolsep{1pt} 
\caption{Share of uncensored DNS responses for probes using ISP resolvers in Germany for domain names removed from the block list by the German regulator.}\label{tbl:overblocking_de} 
\centering 
\scriptsize 
\adjustbox{max width=\textwidth}{% 
\begin{tabular}{l c c c c c } 
 & \DomainHead{2022-08-01} & \DomainHead{2022-10-31} & \DomainHead{2023-02-10} & \DomainHead{2023-07-26} & \DomainHead{2023-09-01} \\ \midrule 
 www.russisches-tv-fernsehen.de & \cellcolor{13} 87 & \cellcolor{15} 98 & \cellcolor{15} 98 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 www.coolstreaming.us & \cellcolor{13} 86 & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
\bottomrule
\end{tabular}}
\end{table}

==> tables/ripe_atlas_dns_sputnikglobe.tex <==
\definecolor{0}{rgb}{0.267004,0.004874,0.329415} 
\definecolor{1}{rgb}{0.282656,0.100196,0.42216} 
\definecolor{2}{rgb}{0.277134,0.185228,0.489898} 
\definecolor{3}{rgb}{0.253935,0.265254,0.529983} 
\definecolor{4}{rgb}{0.221989,0.339161,0.548752} 
\definecolor{5}{rgb}{0.190631,0.407061,0.556089} 
\definecolor{6}{rgb}{0.163625,0.471133,0.558148} 
\definecolor{7}{rgb}{0.139147,0.533812,0.555298} 
\definecolor{8}{rgb}{0.120565,0.596422,0.543611} 
\definecolor{9}{rgb}{0.134692,0.658636,0.517649} 
\definecolor{10}{rgb}{0.20803,0.718701,0.472873} 
\definecolor{11}{rgb}{0.327796,0.77398,0.40664} 
\definecolor{12}{rgb}{0.477504,0.821444,0.318195} 
\definecolor{13}{rgb}{0.647257,0.8584,0.209861} 
\definecolor{14}{rgb}{0.82494,0.88472,0.106217} 
\definecolor{15}{rgb}{0.993248,0.906157,0.143936} 
\begin{table} 
\setlength\tabcolsep{1pt} 
\caption{Share of uncensored DNS responses received by RIPE Atlas probes relying on ISP upstream resolvers for sputnikglobe.com over time.}\label{tbl:blocking_sputnikglobe} 
\centering 
\scriptsize 
\adjustbox{max width=\textwidth}{% 
\begin{tabular}{l c c c } 
 & \DomainHead{2023-04-19} & \DomainHead{2023-07-26} & \DomainHead{2023-09-01} \\ \midrule 
 AT & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 BE & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 BG & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 CH & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 CY & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 CZ & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 DE & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 99 \\ 
 DK & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 EE & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 ES & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 FI & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{1} \color{white} 7 \\ 
 FR & \cellcolor{15} 100 & \cellcolor{15} 99 & \cellcolor{15} 100 \\ 
 GB & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 GR & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 HR & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 HU & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 IE & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 IT & \cellcolor{15} 98 & \cellcolor{15} 98 & \cellcolor{15} 100 \\ 
 LT & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 NL & \cellcolor{15} 100 & \cellcolor{15} 98 & \cellcolor{15} 100 \\ 
 PL & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 PT & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 RU & \cellcolor{15} 100 & \cellcolor{15} 97 & \cellcolor{14} 89 \\ 
 SE & \cellcolor{15} 100 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 SI & \cellcolor{15} 100 & \cellcolor{1} \color{white} 10 & \cellcolor{2} \color{white} 16 \\ 
 SK & \cellcolor{9} 60 & \cellcolor{15} 100 & \cellcolor{15} 100 \\ 
 US & \cellcolor{15} 98 & \cellcolor{15} 98 & \cellcolor{15} 100 \\ 
\bottomrule
\end{tabular}}
\end{table}


